SHMC-Net: A Mask-guided Feature Fusion Network for Sperm Head Morphology Classification

Male infertility accounts for about one-third of global infertility cases. Manual assessment of sperm abnormalities through head morphology analysis encounters issues of observer variability and diagnostic discrepancies among experts. Its alternative, Computer-Assisted Semen Analysis (CASA), suffers from low-quality sperm images, small datasets, and noisy class labels. We propose a new approach for sperm head morphology classification, called SHMC-Net, which uses segmentation masks of sperm heads to guide the morphology classification of sperm images. SHMC-Net generates reliable segmentation masks using image priors, refines object boundaries with an efficient graph-based method, and trains an image network with sperm head crops and a mask network with the corresponding masks. In the intermediate stages of the networks, image and mask features are fused with a fusion scheme to better learn morphological features. To handle noisy class labels and regularize training on small datasets, SHMC-Net applies Soft Mixup to combine mixup augmentation and a loss function. We achieve state-of-the-art results on SCIAN and HuSHeM datasets, outperforming methods that use additional pre-training or costly ensembling techniques.

==> related_works.tex <==
\section{Related Work}
We review some prominent works on sperm head morphology classification and other related problems. 
% \comments{General Sperm papers}:  \\
% \comments{Sperm head papers}: \\ 
% \comments{Sperm morphology papers old CV.}: ~\cite{violetaCESVM},\cite{shakerAPDL}\\
% \comments{Sperm morphology papers DL based.} :\cite{iqbalMCHSH},\cite{liuTL},\cite{lclm-mdl},\cite{riordonFTVGG},\cite{shmcnn} \\
% \comments{segmentation Mask based approaches for classifications}:~\cite{charleyCasa} \\
% \comments{What we are proposing}: \\
% \comments{fusion networks}:~\cite{fusionSCIDS},~\cite{spencer2022ensembled},~\cite{multiModelCNNFusion}\\
% % \comments{gated regularizations}:~\cite{gateRegularizer} \\
% \comments{mixup augmentations}:~\cite{zhang2018mixup}
% Concerning the line of works in automated sperm head morphology classification

\subsection{Sperm Morphology Classification} 
Automating sperm head morphology classification has attracted attention in CV and DL research in the last decade. Previous methods combined hand-crafted shape-based features and traditional machine learning approaches \cite{violetaCESVM,goldScian,shakerAPDL} as a viable alternative for manual assessment of sperm morphology anomalies. 
But, manual feature design is time-consuming, labor-intensive, and may not capture all relevant morphology information in sperm images. 
DL has fueled automated sperm analysis by eliminating the need for hand-crafted features. Several DL methods \cite{riordonFTVGG,liuTL} leveraged 
%the strengths of 
CNNs for better sperm morphology classification. 
%These methods were the immediate applications of CNN architecture advancements on sperm morphology classification tasks. 
%Methods that were catered toward sperm morphology analysis \cite{iqbalMCHSH, shmcnn,ilhan2020automated, lclm-mdl} through 
Some methods \cite{iqbalMCHSH, shmcnn,ilhan2020automated, lclm-mdl} made specific changes on CNN architectures or used strategic data pre-processing or dedicated image feature-learning methods for sperm morphology analysis.
%have also been effective. 

Another line of work used additional pre-training (other than ImageNet) to improve performance, including supervised pre-training on an external dataset \cite{fusionSCIDS} and unsupervised pre-training \cite{charleyCasa} on the same dataset for a downstream classifications task. 
However, pre-training requires additional computation, training time, and hyper-parameter tuning. 
Other methods adopted ensemble techniques~\cite{yuzkat2021multi,spencer2022ensembled} to further boost performance, but with a trade for even higher computation costs and overall model complexity.
% significant performance improvements have come through ensemble techniques \cite{yuzkat2021multi,spencer2022ensembled} but ensembling is computationally costly.

DL-based methods have brought automated sperm morphology analysis of sperm images to new heights, but further improvements are still limited due to the fundamental challenges of such images: low quality, limited quantity, distracted structures, and noisy labels --- these have not been fully addressed in previous works.




% With the advancement and widespread application of deep learning, an increasing number of methods are being utilized for this issue. Jason et al. promoted FT-VGG~\cite{riordonFTVGG}, a highly accurate sperm classification model utilizing the ImageNet pretrained VGG16 network with changed structure at the end of the model. Liu et al.~\cite{liuTL} enhanced the classification network by adding Batch Normalization layers to AlexNet's feature extraction for improved performance. 
% Ni et al. introduced LCLM-MDL~\cite{lclm-mdl}, a model incorporating local constraint and label embedding to capture nonlinear structures and discriminability features. Specialized CNNs like MC-HSH~\cite{iqbalMCHSH} and SHMCNN~\cite{shmcnn} were also designed for sperm head morphology classification. Despite significant improvements, most of these methods rely on minor modifications to the original network, leading to a lack of generalization and robustness.

% Chang et al. employed CE-SVM~\cite{violetaCESVM}, a Cascade Ensemble of Support Vector Machines with various shape descriptors to classify sperm heads. Shaker et al. introduced APDL~\cite{shakerAPDL}, a dictionary learning method using prototype matching of image patches to determine the best matching class based on the lowest reconstruction error from test image patches, while extracting square patches from sperm head images and learning class-specific dictionaries from columnized patches. However, manual feature design is time-consuming, labor-intensive, and may limit classification performance by not capturing all relevant information in complex data. 


% \comments{Based on the previous works, several research works have been dedicated to enhancing performance through various approaches. Spencer et al. presented a stacked ensemble of convolutional neural networks by combining traditional CNN models with modern residual and densely connected architectures using a multi-class meta-classifier~\cite{spencer2022ensembled}. Y{'u}zkat et al.~\cite{yuzkat2021multi} combined six different CNN networks, with two decision-level fusion techniques namely hard-voting and soft-voting, for completely automating the morphological classification process. Further, Ilhan et al. introduced a two-stage framework that employed two pretrained network to classify raw sperm patches by using high level spatial features comprising extreme distinctive ability with soft-voting technique~\cite{ilhanSMIDS}. However, either training multiple models in parallel or two-stage training requires a significant amount of resources and is time-consuming, while fusion at decision-level may result in the loss of feature correlations obtained by different models during training on similar samples. Zhang et al.~\cite{charleyCasa} utilized features from sperm head segmentation masks to guide the model to learn more relevant information, with a two-stage training scheme contains an useful foreground distillation module and a soft-tunning module to refined masks for background denoising. Despite achieving feature-level fusion between segmentation masks and raw sperm images, the two-stage training scheme still demands more resources and time for training, potentially affecting its efficiency. Therefore, in order to leverage the benefits of the mentioned categories fully, a lightweight end-to-end framework with feature-level fusion becomes necessary.}

\subsection{Sperm Cell Segmentation}
Traditional CV methods have been applied to obtain reasonable sperm cell segmentation masks 
using ellipse fitting \cite{park1997segmentation,nafisi2005sperm}, thresholding and clustering \cite{carrillo2007computer,vchang2014goldSeg}, or combinations of the above \cite{charleyCasa, ilhan2019automaticEllep}. 
These methods are usually effective but may generate masks with imperfect boundaries. 
DL-based methods
\cite{movahed2018learning,nissen2017convolutional,mashaal2022automatic,lv2022improved} have gained popularity in generating sperm masks in a supervised fashion, but they require training data which may be too costly to obtain in many applied cases. 
Zhang et al.~\cite{charleyCasa} proposed a hierarchical pseudo-mask (HPM) generation method to obtain reliable sperm head segmentation masks using the size, shape, contrast, location, and data priors within the sperm images, and further refined the mask boundaries using a DL component. 
However, the DL-based mask refinement component is an overhead for such a classification network. 
As an alternative, we adopt graph-based boundary refinement methods that are ubiquitous \cite{liangRegistrationGraphSearch, falcao2004imageGS,li2005optimalGS3D, Jwang2015segmenting} and widely used in medical image analysis for both 2D images and 3D volumes. 
We present a simple graph-based method for sperm head mask refinement in Section~\ref{Mask Generation}.
% While their method shows the effectiveness of using segmentation masks for unsupervised pre-training to facilitate the downstream task of head morphology classification, a more explicit use of the segmentation mask could further elevate the morphology classification.

\subsection{Feature Fusion}

The idea of fusing features has been widely used in DL research \cite{inceptionNet, resnet, unet} for capturing different feature granularities at multiple scales or training extremely deep networks. 
In biomedical image analysis, fusion schemes have been proposed \cite{tchenFusion,ttchenFusion2022,cpeng2022imiin} to use multi-modal data for improved classification or segmentation. 
We apply feature fusion to make effective use of the mask information to guide the classification network, 
%and suggest the experiments-backed appropriate fusion scheme (section \ref{fusion_scheme}), 
exploiting features of the sperm images and segmentation masks. 
    
\subsection{Mixup Augmentation}
Mixup augmentation \cite{zhang2018mixup} is one of the common regularization processes to prevent overfitting by feeding a DL model with linearly interpolated samples and labels. 
One of the commonly-used mixup approaches, inter-class mixup \cite{yun2019cutmix},\cite{zhao2023tokenmix},\cite{uddin2020saliencymix}, involves mixing the input data of two different classes during training, but this might dilute the features by mixing characteristics from different classes. Alternatively, intra-class mixup \cite{zhao2021intra},\cite{zhang2021intra},\cite{hendrycks2019augmix} 
%has been suggested that 
involves mixing the input data within the same class, and thus preserves class characteristics and handles intra-class variations. 
Previous works \cite{balancedmixup} have demonstrated that combining mixup with sampling techniques effectively addresses class imbalance problems. We combine intra-class mixup, oversampling, and a carefully designed loss function to handle the problems of noisy labels and class imbalance prevalent in sperm datasets. 

% method~\cite{zhang2018mixup}
% Intra Mixup: \cite{zhao2021intra}, \cite{intraClassMixup}, \cite{zhang2021intra}, \cite{hendrycks2019augmix}
% Inter Mixup: \cite{yun2019cutmix}, \cite{uddin2020saliencymix}, \cite{zhao2023tokenmix}







